Continuous Embedding Attacks via Clipped Inputs in Jailbreaking Large Language Models

Security concerns for large language models (LLMs) have recently escalated, focusing on thwarting jailbreaking attempts in discrete prompts. However, the exploration of jailbreak vulnerabilities arising from continuous embeddings has been limited, as prior approaches primarily involved appending discrete or continuous suffixes to inputs. Our study presents a novel channel for conducting direct attacks on LLM inputs, eliminating the need for suffix addition or specific questions provided that the desired output is predefined. We additionally observe that extensive iterations often lead to overfitting, characterized by repetition in the output. To counteract this, we propose a simple yet effective strategy named CLIP. Our experiments show that for an input length of 40 at iteration 1000, applying CLIP improves the ASR from 62% to 83%

==> tex/Discussion.tex <==
\section{Discussion}
We observe that longer input lengths corresponded to lower ASR@K accuracy.
We also observed that longer lengths have lower initial loss than length 1. Additionally, longer lengths allow the model to leverage more information to minimize the loss, sometimes at the cost of sacrificing the model's ability to generalize. These two factors lead to a more drastic decrease in loss for longer lengths, thereby causing quicker overfitting.
Additionally, we explored the impact of $\alpha$. Without \tool{}, the Frobenius norm of the input increased, sometimes causing numerical instability. Implementing \tool{} stabilized this metric, but it may be hard to approximate the target output in constrained subspaces with limited information, like length 1, and therefore require a loose $\alpha$ in Algorithm~\ref{alg:1}.
